SFT or RL? An Early Investigation into Training R1-Like Reasoning Large Vision-Language Models

This work revisits the dominant supervised fine-tuning (SFT) then reinforcement learning (RL) paradigm for training Large Vision-Language Models (LVLMs), and reveals a key finding: SFT can significantly undermine subsequent RL by inducing ``pseudo reasoning paths'' imitated from expert models. While these paths may resemble the native reasoning paths of RL models, they often involve prolonged, hesitant, less informative steps, and incorrect reasoning. To systematically study this effect, we introduce VLAA-Thinking, a new multimodal dataset designed to support reasoning in LVLMs. Constructed via a six-step pipeline involving captioning, reasoning distillation, answer rewrite and verification, VLAA-Thinking comprises high-quality, step-by-step visual reasoning traces for SFT, along with a more challenging RL split from the same data source. Using this dataset, we conduct extensive experiments comparing SFT, RL and their combinations. Results show that while SFT helps models learn reasoning formats, it often locks aligned models into imitative, rigid reasoning modes that impede further learning. In contrast, building on the Group Relative Policy Optimization (GRPO) with a novel mixed reward module integrating both perception and cognition signals, our RL approach fosters more genuine, adaptive reasoning behavior. Notably, our model VLAA-Thinker, based on Qwen2.5VL 3B, achieves top-1 performance on Open LMM Reasoning Leaderboard (https://huggingface.co/spaces/opencompass/Open_LMM_Reasoning_Leaderboard) among 4B scale LVLMs, surpassing the previous state-of-the-art by 1.8%. We hope our findings provide valuable insights in developing reasoning-capable LVLMs and can inform future research in this area.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> others/TBD.tex <==
\subsection{Effect of SFT on GRPO Training}

Although we reveal in Section~\ref{sec:revisit_sft_role} that SFT alone leads to a performance drop on multimodal reasoning tasks, it is still unclear whether SFT plays a crucial role in aiding GRPO, like the golden key in DeepSeek-R1.
We thus conduct experiments to ablate for the effect of SFT before GRPO.
% reasoning like the common practice in DeepSeek-R1 remains underexplored.
% it is not yet clear whether SFT helps GRPO training. 
% Therefore, it is crucial to ablate for the effect of SFT before we can determine the final training recipe.





\subsubsection{Choices of Backbones for GRPO}

% \begin{figure*}[ht]
% \centering
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \begin{tabular}{ll}
%     \toprule
%     GRPO Backbone & Avg. Perf. \\ 
%     \midrule
%     Qwen2-VL-2B & 20.3 \\ 
%     Qwen2-VL-2B + SFT & 17.7 \\ 
%     Qwen2-VL-Base-2B + SFT & 17.5 \\ 
%     Qwen2-VL-Base-2B & 0.0 \\
%     % Qwen2-VL-Base-2B & 0.0\textcolor{red}{~\tiny\raisebox{-0.5ex}{(–100\%)}} \\ 
%     \midrule
%     Qwen2-VL-7B & 32.5 \\ 
%     Qwen2-VL-Base-7B & 30.7 \\ 
%     Qwen2-VL-Base-7B + SFT & 25.7 \\ 
%     Qwen2-VL-7B + SFT & 19.8 \\ 
%     \bottomrule
%     \end{tabular}
%     \captionof{table}{Performance of GRPO training on different backbones.}
%     \label{tab:inst_following}
% \end{minipage}
% \hfill
% \begin{minipage}{0.48\textwidth}
%     \centering
%     \includegraphics[width=\linewidth]{figs/hidden_states_geoqa170k.pdf}
%     \caption{Hidden states of Qwen2VL-7B family before and after GRPO training on different backbones.\hardy{what conclusion?}}
%     \label{fig:sft_hidden_states_geoqa170k}
% \end{minipage}

% \end{figure*}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{figs/hidden_states_geoqa170k.pdf}
%     \caption{Hidden states of Qwen2VL-7B family before and after GRPO on difference backbones.}
%     \label{fig:sft_hidden_states_geoqa170k}
% \end{figure}


% \begin{table}[ht]
% \centering
% % \small
% \begin{tabular}{llc}
% \toprule
% GRPO Trained on & Avg. Perf. \\ \midrule
% Qwen2-VL-2B & 20.3 \\ 
% Qwen2-VL-2B + SFT & 17.7   \\ 
% Qwen2-VL-Base-2B + SFT & 17.5 \\ 
% Qwen2-VL-Base-2B & 0.0\textcolor{red}{~\tiny\raisebox{-0.5ex}{(–100\%)}} \\ 
% \midrule
% Qwen2-VL-7B & 32.5 \\ 
% Qwen2-VL-7B + SFT &   \\ 
% Qwen2-VL-Base-7B + SFT &  \\ 
% Qwen2-VL-Base-7B & 30.7 & \\ 
% \bottomrule
% \end{tabular}
% \caption{Performance of GRPO training on different base models. }
% \label{tab:inst_following}
% \end{table}


We experiment with different backbones for GRPO training. Specifically, we adopt Qwen2VL-7B-Base and Qwen2VL-7B-Inst, and perform SFT on them with 25K samples.
We then perform GRPO on the four backbones and compare their performance.
% eval
For evaluation, we check the token distributions for each setting. We randomly choose 100 samples from each source of \grpods, totaling 900 samples, prompt each model for generation, and compute the observed token distribution.


\begin{table}[ht]
\centering
\begin{tabular}{l|cc}
\toprule
SFT/GRPO Backbone & KL Div. with *+SFT & KL Div. with *+GRPO \\
\midrule
Qwen2VL-7B-Base      & 0.99 & 0.81 \\
Qwen2VL-7B-Inst      & 1.35 & 0.81 \\
Qwen2VL-7B-Base+SFT  & --   & 0.27 \\
Qwen2VL-7B-Inst+SFT  & --   & 0.25 \\
\bottomrule
\end{tabular}
\caption{\small KL divergence on token distributions before and after SFT/GRPO with different backbones.
For the first column, 
0.99 is the KL divergence between \textit{Qwen2VL-7B-Base} and \textit{Qwen2VL-7B-Base-SFT}.
1.35 is the KL divergence between \textit{Qwen2VL-7B-Inst} and \textit{Qwen2VL-7B-Inst-SFT}.
}
\label{tab:sft_vs_grpo_output_ids_distribution_kl}
\end{table}


% \paragraph{GRPO has less impact in shifting token distributions on SFTed models.} 
\paragraph{SFT Memorizes Pseudo Reasoning paths on which GRPO Fails to Improve.}

Table~\ref{tab:sft_vs_grpo_output_ids_distribution_kl} summarizes the KL divergence brought by SFT/GRPO training. Note that since all models share the same vocabulary, their KL divergence values are comparable.
Comparing the numbers in the top two rows, SFT shifts distributions more than GRPO does, on both Base and Inst backbone. 
These results add to previous ones and show that SFT can cause considerable changes in token distribution, and such changes are harmful to the reasoning ability of LVLMs since models only learn pseudo reasoning paths. 
Meanwhile, comparing the numbers in the second column, GRPO results in a KL of 0.81 on non-SFTed backbones, and less than 0.3 on the SFTed ones.
This suggests that once the pseudo reasoning patterns are learned, it would be hard for the model to acquire the genuine reasoning ability via GRPO. 








% \begin{table}[ht]
% \centering
% \begin{tabular}{c|cccc}
% \toprule
% \multirow{2}{*}{SFT Backbone} & \multicolumn{4}{c}{\textit{Qwen2VL-7B Family}}\\
%  & \multicolumn{2}{c}{Base}   & \multicolumn{2}{c}{Inst}   \\ \midrule
% KL Div. with *+SFT & \multicolumn{2}{c}{0.99} & \multicolumn{2}{c}{1.35}\\
% \midrule
% \midrule
% \multirow{2}{*}{GRPO Backbone} & \multicolumn{4}{c}{\textit{Qwen2VL-7B Family}}\\
%  & Inst & Base & Base+SFT & Inst+SFT \\ \midrule
% KL Div. with *+GRPO & 0.81 & 0.81 & 0.27 & 0.25 \\
% \bottomrule
% \end{tabular}
% \caption{\small KL divergence on token distributions before and after GRPO with different backbones.}
% \label{tab:sft_vs_grpo_output_ids_distribution_kl}
% \end{table}








\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/output_ids_all.pdf}
    \caption{Distribution and cumulative probability of top-15 tokens from responses of Qwen2VL-7B family. 
    Inst: Qwen2VL-7B-Instruct; 
    Base: Qwen2VL-7B-Base; 
    Base+SFT: SFT on Qwen2VL-7B-Base; 
    Inst+SFT: SFT on Qwen2VL-7B-Instruct.
    Blue bars are the observed token probability sorted by descending frequency with scale shown on the left y-axis.
    Red dots are cumulative probability with scale shown on the right y-axis.
    The overall entropy from all tokens is shown below each title.
    For the lower row, average benchmark performances are shown.}
    \label{fig:sft_vs_grpo_output_ids_distribution}
\end{figure}
% \paragraph{Benchmark performance is roughly consistent with the cumulative probability of frequent tokens.}
\paragraph{GRPO Works by Finding Effective Reasoning Paths, rather than creating new ones.}
We compute the overall entropy of each distribution and plot the (cumulative) probability of the most frequent 15 tokens in Figure~\ref{fig:sft_vs_grpo_output_ids_distribution}.
Comparing Inst with Inst+SFT, and Base with Base+SFT, we find that SFT shifts the distribution towards a more uniform one, indicated by the increased entropy. In contrast, comparing the upper and lower row, GRPO barely changes the uniformness of distribution. This result aligns with~\citep{kirk2023understanding} which finds that outputs from RLHFed models are less diverse than SFTed models.
However, in terms of benchmark performance, Inst+GRPO outperforms the rest with the smallest entropy among all.
These observations may indicate that GRPO works by finding effective reasoning paths in a given number of paths, rather than creating new paths, and that the pseudo paths learned by SFT indeed introduce difficulty for GRPO to find truly effective ones.


% % guess
% Although xx reveal that 



% \paragraph{GRPO only requires to start on a model with decent instruction following ability}
% \paragraph{Better Instruction-following $+$ GRPO $\rightarrow$ Better Reasoning.} 
% \paragraph{Better General Instruction-following $+$ GRPO $\rightarrow$ Better Reasoning.} 
% \hardy{discard?}
% Unlike previous research on reasoning models that emphasizes format-following in the initial phase, we discover that the key to RL's success lies in its ability to follow \textit{general instructions}, rather than \textit{task-specific instructions}.




\subsubsection{Scaling Down SFT Data}
\begin{figure}[ht]
% \vspace{-30pt}
    \centering
    \includegraphics[width=.8\linewidth]{figs/min_sft_data_benchmarks_v0.1.pdf}
    \caption{Impact of SFT with 5K and 10K samples before GRPO.}
    \label{fig:sft_5k_vs_10k}
\end{figure}

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/min_sft_data_wandb_log.pdf}
    \caption{Comparison of response length and reward during training.}
    \label{fig:sft_grpo_length_and_reward}
\end{figure}

Since we reveal in Section~\ref{sec:sft_findings} that more SFT data yields lower performance, we try to investigate the effect of downsizing the SFT training set.
% setting
Following the PPL filtering method in Section~\ref{sec:revisit_sft_role}, we select top-10K and top-5K samples from \sftds\ to finetune Qwen2.5-VL-3B, followed by GRPO training. For comparison, we also conduct GRPO training without SFT.  

% \paragraph{More SFT Data Further Degrades GRPO Performance.}
\paragraph{Smaller SFT dataset still jeopardizes GRPO performance.}
% We present performance of Qwen2.5-VL-3B on each task in Figure~\ref{fig:enter-label}. 
% The direct finding is that SFT on 5K data before GRPO largely compromises the model performance compared to just GRPO --- average 13.5\% drop over 6 math benchmarks.
% Also, when pre-trained on more SFT data, the performance does not change significantly by a slightly improvements of 0.8\%.
% These findings further verify that the training paradigm of SFT is not the best practice for teaching thinking of LVLMs, it even adversely impact its inherent learning abilities. 
% findings
We present the performance of Qwen2.5-VL-3B on each task in Figure~\ref{fig:sft_5k_vs_10k}. 
A clear observation is that applying SFT on 5K examples prior to GRPO significantly degrades performance compared to using GRPO alone, showing an average drop of 13.5\%. 
Moreover, scaling up SFT data to 10K yields only a marginal improvement of 0.8\%. 
These results further support that SFT before GRPO can hinder the model's learning capability. 
% These results further support the claim that SFT is not an optimal paradigm for teaching self-reasoning in LVLMs. 
% In fact, it may even hinder the model’s inherent learning capabilities.

\textbf{Response length, reward, and model performance are NOT necessarily related.~~}
\hardy{add contradiction of conclusion of previous studies}
Existing researches in RL suggest a correlation between 
Figure~\ref{fig:sft_grpo_length_and_reward} shows that the model response length and reward in GRPO are not reliable indicators of reasoning ability.
The 10K SFT+GRPO model generates the longest responses but yields lower rewards than GRPO-only ($\sim$0.35 \vs $\sim$0.5) at the end of training . 
Similarly, 5K SFT+GRPO achieves moderate length and reward but underperforms in downstream tasks.

Interestingly, both SFT-ed models start with higher initial rewards (\eg, $\sim$0.20 for 10K SFT+GRPO \vs $\sim$0.05 for GRPO-only), which is likely due to their early learning experience with supervision since SFT and GRPO data share the same distribution. 
However, they exhibit limited reward improvement during training, whereas the GRPO-only model rapidly surpasses them.
These trends further reveal that SFT solely provides a higher ``lower bound'' for RL training, yet it may lower the ``upper bound'' since the reasoning SFT data constrains the model's exploration paths.
Therefore, \textbf{reasoning is a native emerging ability that is more likely to be developed through RL, not SFT}. 
While SFT-ed models may appear to reason, their behavior is closer to pattern imitation --- \textbf{a form of pseudo-reasoning that lacks the generalizable reasoning skills}.

% Another interesting observation during training is that, latex format

% $\Rightarrow$ {\color{red}{pseudo-reasoning (via SFT) VS native reasoning (via RL); reasoning is an emerging ability acquired via RL.}}
% \begin{enumerate}

% \item sft for answer format learning
%     \begin{enumerate}
%         \item design a minimal set of sft data such that the model is able to follow answer format: 128k $\rightarrow$ 25K $\rightarrow$ 10K $\rightarrow$ 5K $\rightarrow$ 1024 $\rightarrow$ 512 ) for format learning, and show that this is better than not using any instruction data.
%         \item Show that sft is not critical for GRPO training when model is already capable of following instructions (qwen2vl-base, qwen2vl-instruct, qwen25vl)
%     \end{enumerate}
% \end{enumerate}

% \section{Discussion}
% Discussion: Pseudo reasoning (learned via sft) VS native reasoning (learned via RL). length isn't everything.
% compare length of generation \haoqin{I added some discussions, need double-check}


